Bridging HPC and Quantum Systems using Scientific Workflows

Quantum Computers offer an intriguing challenge in modern Computer Science. With the inevitable physical limitations to Moore's Law, quantum hardware provides avenues to solve grander problems faster by utilizing Quantum Mechanical properties at subatomic scales. These futuristic devices will likely never replace traditional HPC, but rather work alongside them to perform complex tasks, utilizing the best of decades of HPC and quantum computing research. We leverage the capabilities of scientific workflows to make traditional HPC and Quantum Computers work together. To demonstrate this capability, we implemented three algorithms: Grover's Search Algorithm, Shor's Factoring Algorithm, and a 4-node Traveling Salesman Algorithm. The algorithms' implementation and generated inputs are sent from ORNL HPC to IBMQ, the algorithms run on IBMQ, and the results return. The entire process is automated as a workflow by encoding it into the Parsl parallel scripting and workflow platform.

==> __latexindent_temp.tex <==
This research used resources of the Oak Ridge Leadership Computing Facility at the Oak Ridge National Laboratory, which is supported by the Office of Science of the U.S. Department of Energy under Contract No. DE-AC05-00OR22725.

==> abstract/abstract.tex <==
\begin{abstract}
Quantum Computers offer an intriguing challenge in modern Computer Science. With the inevitable physical limitations to Moore's Law, quantum hardware provides avenues to solve grander problems faster by utilizing Quantum Mechanical properties at subatomic scales. These futuristic devices will likely never replace traditional HPC, but rather work alongside them to perform complex tasks, utilizing the best of decades of HPC and quantum computing research. We leverage the capabilities of scientific workflows to make traditional HPC and Quantum Computers work together. To demonstrate this capability, we implemented three algorithms: Grover's Search Algorithm, Shor's Factoring Algorithm, and a 4-node Traveling Salesman Algorithm. The algorithms' implementation and generated inputs are sent from ORNL HPC to IBMQ, the algorithms run on IBMQ, and results return back. The entire process is automated as a workflow by encoding it into the Parsl parallel scripting and workflow platform.
\end{abstract}

\begin{IEEEkeywords}
HPC, quantum computing, workflows
\end{IEEEkeywords}


==> abstract/sec-algorithms.tex <==
\section{Quantum Algorithms}

In this section we discuss our experience constructing and then running the three aforementioned algorthms over real Quantum Computing Systems using the Qiskit library~\cite{Qiskit} orchestrated remotely from OLCF HPC. Full results, along with results for the following algorithms, are available in the project GitHub Repository~\cite{Bieberich_HPC-QC-Workflows_2022}. We implemented the algorithms as part of a scientific workflow using the Parsl~\cite{10.1145/3307681.3325400} parallel scripting and workflow platform, which allows for the implicit parallelization among internal tasks based on data and control dependencies. 



\subsection{Grover's Algorithm}

Grover's algorithm allows for one to find an item in an unsorted list of N length using $O(\sqrt{N})$ operations, as opposed to $O(N)$ operations on average for a classical computer~\cite{adedoyin2018quantum}. The Algorithm is split into three steps, first being initialization, followed by the Grover operation, then measurement. It is most accurate when the Grover operator is repeated $\sqrt{N}$ times, where $N$ is the number of qubits.

\paragraph*{Results}
We designed the quantum circuit and the rest of the program in with the IBMQ library Qiskit~\cite{ibm-quantum}. The program randomly chose a number between 0 and 15. Once this number was chosen, it was printed and saved as a variable (to compare with results), and then a loop created the unique Grover Oracle. Next, the circuit was sent to IBM's ibmq-belem 5-qubit Quantum Computer. After 1024 shots of the circuit, the results are sent back to the supercomputer, which makes a histogram displaying the results. On average, 92\% of the shots returned the number input.    

\subsection{Shor's Algorithm}

More than any other Quantum Algorithm, Peter Shor's Factoring Algorithm~\cite{365700} has created the most buzz. Currently prevalent RSA encryption techniques are composed of keys made of the factors of RSA-2048, a 2048-bit number. It is almost impossible to find the prime factors of such large numbers with classical computing which Shor's algorithm promises to find.

Shor's Algorithm is composed of a series of steps based on an algorithm that has long been theorized, but is difficult to implement at a large scale on regular computers: the Period Finding Problem. The Period Finding Problem states that there exists an $r$ such that $x^r\mod{}N = 1$, leading to the greatest common divisor of $x^{r/2}\pm1$ and $N$ being one of the prime factors~\cite{vazirani_2004}. Using the period finding problem function on a Quantum Computer, RSA-2048 and other large semi-primes could be factorable, although thousands of qubits would be needed to implement this program for such a large number.

\paragraph*{Implementation}

The circuit for Shor's Algorithm that we used uses two qubit registers, one that encompasses 0-2 qubits, called the ``work register'', and the second encompassing qubits 3-6, called the ``control register''. The circuit for Shor's Algorithm can be broken into four distinct sections: Initialization, Modular Exponentiation, Inverse Quantum Fourier Transform (QFT), and Measurement. In the Initialization step, all three qubits in the work register are put into superposition, and a NOT gate is applied to the final qubit in the control register. The Modular Exponentiation stage uses $U^{2^j}$ gates to perform a Quantum Phase Estimation on the three work register qubits, resulting in the work register ending in a state $a^x\mod{}N$. The Inverse QFT takes these values and creates interference between the states, turning the current circuit value and converting it to a Fourier basis~\cite{amico2019experimental}. Lastly, the work register qubits are measured. 

\paragraph*{Results}

The larger a circuit is, the more computational time it takes to run and thus more noise is exposed to the delicate qubits running the operations. Thus, the results become further from the expected values, as opposed to the smaller Grover circuit. Tests on IBM's Quantum Computers provided no conclusive results. In contrast, the simulator outputs an almost perfect four-way distribution of the measured counts: 0, 2, 4, and 6, in binary. The way the circuit was designed, 0 always features a large distribution, and is thus ``ignored", but the following values, 2, 4, and 6, exhibit the period of the function. 


\subsection{The 4-Node Traveling Salesman Problem Algorithm}

\paragraph*{Problem Description}

The Traveling Salesman Problem (TSP) is a well-known optimization problem with significant implications. The TSP asks for the shortest path between $N$ cities (or nodes), assuming you start and end at the same city. This results in $(N-1)!$ different routes that may be taken. While there are many algorithms to solve TSP implementations with relatively few nodes, even supercomputers are unable find the best distance with hundreds of nodes in polynomial time~\cite{dahiya_sangwan_2018}. 

\paragraph*{Creating the Algorithm}

\begin{figure}
    \includegraphics[scale = 0.27]{figs/tsp-map.png}
    \caption{NetworkX network map for 4 node Traveling Salesman Problem.}
    \label{fig:map}
\end{figure}

\begin{figure*}[b!]
    \includegraphics[scale = 0.4]{figs/1-2-3-4-on-qasm.png}
    \caption{1-2-3-4 path Traveling Salesman Problem circuit results from IBMQ's Cloud QASM.}
    \label{fig:qasm}
\end{figure*}

Much of the process for designing the TSP 4-node circuit is from the Qiskit Alpha Textbook~\cite{Qiskit-Textbook}, which utilized Phase Estimation. The algorithm we used utilized distance matrices converted to phases. After getting unitary matrices for each of the four nodes, these can be converted to high-level gates in a Quantum algorithm. A concurrent step involves determining the Eigenstates. As mentioned before, there are $(N-1)!$ paths in a TSP, where $N$ is the number of nodes being tested. Each path can be mapped to a unique Eigenstate in binary.

To further optimize the program, it can be proven that the paths 1-2-3-4-1 and 1-4-3-2-1 are the same; thus, the number of Eigenstates can be reduced to $(N-1)!/2$, or 3 for a four-node TSP. 

\paragraph*{Hybrid Workflow Explained}

After loading credentials, the rest of the code was split into five main steps:

\begin{enumerate}
    \item The code, via the ``random" and ``networkx'' functions, creates random coordinates for each of the four nodes and then graphs them~\cite{hagberg2008exploring}. A file similar to Fig. \ref{fig:map} is created on the local computer.
    \item A second Python function reads the coordinates from the map and finds the distances between each node, then puts them into a distance matrix.
    \item The quantum circuit is built via Qiskit, including the inverse QFT, which was automatically produced from the Qiskit library in the TSP program. 
    \item The three circuits are sent together, as a Python list, to IBMQ. 
    \item The outputs are read via two variables: the most frequent counts are determined, and functions find which path is the shortest. The results are printed in the supercomputer terminal.
\end{enumerate}

The NetworkX map process takes several seconds, so we organized it to run concurrently (using Parsl) with the Quantum circuit initialization. We were able to run the circuit on the IBMQ QASM simulator and ibmq\_kolkata Quantum Computer at the same time, allowing for predictive results from the simulator to generate as the circuit waits in the queue for the real Quantum Computer.

\paragraph*{Results}

The results are printed as binary strings that are 6 digits long (one for each qubit). Due to the nature of the Phase Estimation, the largest numbers represent the shortest paths that may be taken. For example, in one test we ran, the largest value was 35, which was returned from circuit one, associated with Eigenstate 11000110, or 1-2-3-4-1.

In terms of measured results, we tested the circuit first through IBMQ's ibmq\_kolkata 27 qubit cloud Quantum Computer, then via IBMQ's ibmq\_qasm\_simulator, which can operate up to 32 qubits. The real Quantum Computer featured a significant amount of noise, rendering the results inconclusive. Due to the size of the circuit, too much noise was likely introduced, resulting in significant error. 

On the other hand, the ibmq\_qasm\_simulator proved to offer much more accurate results, as exhibited in Fig.~\ref{fig:qasm}. The reason these results were more accurate has to do with the composition of the QASM simulator. The QASM simulator is run on a classical computer via the Cloud, and while it does model noise, it supports all of the gates in the circuit we wrote, meaning the compiler step does not need to split the CU gates as extensively as ibmq\_kolkata. It also ignores the calibration issues that modern Quantum Computers need, and assumes that all gates are connected, decreasing gate count by several magnitudes.  

==> abstract/sec-conclusion.tex <==
\section{Conclusions}
In this work, we successfully demonstrate the practicality and ease of access to combining classical HPC and Remote Quantum Resources with the help of scientific workflows. In an effort towards a future where Quantum resources may be increasingly available, this work has been a promising preparatory step. Grover's Algorithm, Shor's Algorithm, and the Traveling Salesman Problem are only a few of the many examples that could one day verify Quantum advantage, opening doors to a new scale of research. While Quantum Computers lack the proper hardware to run sufficiently large algorithms, Quantum Software allows for easy access to remote machines and offers hope for optimal HPC and Quantum jobs in the future. Likewise, research in Quantum Error Correction has peaked in recent years, foreshadowing further optimization in new Quantum processors, allowing for larger circuits to run with less error, creating results more on par with the simulators used in this project~\cite{Roffe_2019}. 
%As a continuation of this work, we intend to package the work in the form of a reusable library to explore generic remote Quantum resources.


==> abstract/sec-introduction.tex <==
\section{Introduction}
 
In 1965, Gordon Moore proposed Moore's Law, stating that the number of transistors on a computer chip double every two years, while the price for the same chip is halved~\cite{tardi2021moore}. Recently, Moore's Law has neared its physical limits, as transistors now border the size of single atoms. While this seems to foreshadow grave consequences in High Performance Computing (HPC), discoveries in Quantum Mechanics have promised an abundance of computing power in the future~\cite{abundance}. Quantum computers use Quantum Bits or ``qubits'' that take advantage of Quantum Mechanical phenomena, including superposition and entanglement, which allow for quantum algorithms to offer exponential speedups compared to conventional computers.

Considering how idealized Quantum Computers seem, they do have limitations. HPC has been optimized over the years to solve many problems, but it cannot scale with the same potential as Quantum Computers for a certain class of problems. Quantum Computers, likewise, are unable to solve all computational problems, but are very efficient for many of those which classical computers cannot solve. Furthermore, combining these two resources can allow for significant speedups in many applications, and offer relief for the end of Moore's Law. This work aims to confirm these applications of Quantum Computing, and combine prominent algorithms in Quantum with the classical HPC systems of the Oak Ridge Leadership Computing Facility (OLCF) at Oak Ridge National Laboratory (ORNL). We employ the scientific workflows paradigm~\cite{workflows} to bridge the gap between HPC and Quantum Computers. In particular, we implement three such cases where popular Quantum algorithms receive their inputs from supercomputers over a workflow orchestrated campaign: Grover's Search, Shor's Factorization, and the Traveling Salesman Problem (Fig.~\ref{fig:workflow}).

\begin{figure*}[!t]
    \includegraphics[scale = 0.5]{figs/workflow.png}
    \caption{Overall workflow representation between HPC and Quantum}
    \label{fig:workflow}
\end{figure*}

